Causal Retrieval with Semantic Consideration

Recent advancements in large language models (LLMs) have significantly enhanced the performance of conversational AI systems. To extend their capabilities to knowledge-intensive domains such as biomedical and legal fields, where the accuracy is critical, LLMs are often combined with information retrieval (IR) systems to generate responses based on retrieved documents. However, for IR systems to effectively support such applications, they must go beyond simple semantic matching and accurately capture diverse query intents, including causal relationships. Existing IR models primarily focus on retrieving documents based on surface-level semantic similarity, overlooking deeper relational structures such as causality. To address this, we propose CAWAI, a retrieval model that is trained with dual objectives: semantic and causal relations. Our extensive experiments demonstrate that CAWAI outperforms various models on diverse causal retrieval tasks especially under large-scale retrieval settings. We also show that CAWAI exhibits strong zero-shot generalization across scientific domain QA tasks.

==> table/passage_semanticencoder.tex <==
\begin{table}[hbt!]
  \caption{\textbf{The Accuracy using Semantic encoder as passage encoder.} Task 1 involves retrieving the corresponding effect sentence given a query (cause), while Task 2 is the reverse, retrieving the corresponding cause sentence given the effect.}
  \label{semantic_encoder}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
    \toprule
    Passage encoder
    & \multicolumn{3}{c}{e-CARE} & \multicolumn{3}{c}{e-CARE + CoLA} & \multicolumn{3}{c}{e-CARE + $\text{wiki}_{S}$} & \multicolumn{3}{c}{e-CARE + $\text{wiki}_{M}$}  \multicolumn{3}{c}{e-CARE + $\text{wiki}_{L}$} \\
    \cmidrule(r){2-16}
     & Hit@1 &Hit@10& MRR@10 & Hit@1 &Hit@10& MRR@10 & Hit@1 &Hit@10& MRR@10 & Hit@1 &Hit@10& MRR@10 & Hit@1 &Hit@10& MRR@10 \\
    \midrule
    \multicolumn{16}{c}{Task 1. Cause to Effect} \\
    \midrule
    Semantic encoder
    &0.283 &0.550 &0.362
    & 0.261& 0.512& 0.335 
    & 0.233&0.457 & 0.300 
    & 0.177&0.349 &0.226 
    & 0.124& 0.234 & 0.157 
    \\
    \midrule
    \multicolumn{16}{c}{Task 2. Effect to Cause} \\
    \midrule
    Semantic encoder 
    &0.293 &0.570 &0.372
    & 0.272& 0.524& 0.346 
    & 0.238& 0.484& 0.310 
    & 0.180&0.363 & 0.233 
    & 0.125&0.241 & 0.157
     \\
    \bottomrule
  \end{tabular}}
\end{table}

